Towards Multi-robot Exploration: A Decentralized Strategy for UAV Forest Exploration

Efficient exploration strategies are vital in tasks such as search-and-rescue missions and disaster surveying. Unmanned Aerial Vehicles (UAVs) have become particularly popular in such applications, promising to cover large areas at high speeds. Moreover, with the increasing maturity of onboard UAV perception, research focus has been shifting toward higher-level reasoning for single- and multi-robot missions. However, autonomous navigation and exploration of previously unknown large spaces still constitutes an open challenge, especially when the environment is cluttered and exhibits large and frequent occlusions due to high obstacle density, as is the case of forests. Moreover, the problem of long-distance wireless communication in such scenes can become a limiting factor, especially when automating the navigation of a UAV swarm. In this spirit, this work proposes an exploration strategy that enables UAVs, both individually and in small swarms, to quickly explore complex scenes in a decentralized fashion. By providing the decision-making capabilities to each UAV to switch between different execution modes, the proposed strategy strikes a great balance between cautious exploration of yet completely unknown regions and more aggressive exploration of smaller areas of unknown space. This results in full coverage of forest areas of variable density, consistently faster than the state of the art. Demonstrating successful deployment with a single UAV as well as a swarm of up to three UAVs, this work sets out the basic principles for multi-root exploration of cluttered scenes, with up to 65% speed up in the single UAV case and 40% increase in explored area for the same mission time in multi-UAV setups.

==> tex/backup/05_experiments_backup.tex <==
\section{Experiments}
\label{ch:experiments}
%
We evaluate the proposed exploration pipeline in both single- and multi-robot setups in simulation.
%
In particular, we benchmark our method on a series of realistic, randomly generated forests of increasing tree densities \cite{oleynikova2016continuous}, as well as on a 3D reconstruction of a real forest \cite{afzal2021swarm}. 
%

%
In the single-agent setup, we compare the proposed method against FUEL \cite{zhou2021fuel}, while in the experiments with multiple robots we test against a %we show how our method can reach comparable performance with respect to a 
centralized strategy based on map-splitting.
%, as the best possible alternative given the lack of any relevant decentralized strategies to compare against in the literature.
%
In all tests, we use grid map resolutions of $\SI{0.10}{\meter}$ or $\SI{0.15}{\meter}$ depending on the map size, while we set the dynamic limits to $v_{max} = \SI{1.5}{\meter / \second}$ and $\dot{\gamma}_{max} = \SI{0.9}{rad / \second}$ for all planners.
%
%The main parameters used in the experiments are reported in Table \ref{tab:exp:params}.
%
We simulate a depth camera with a fixed range of $\SI{4.5}{\meter}$ using the Vulkan-based renderer of \cite{bartolomei2022multi} and the same physical simulator as in \cite{zhou2021fuel}. 
%
We report the planners' performance in terms of the time needed to complete the exploration of the scene, the total traveled distance, and the average velocity of the UAVs during each experiment.
%
% \begin{table}
% 	\renewcommand{\arraystretch}{1.1}
% 	\centering
% 	\resizebox{0.5\textwidth}{!}{
% 		\begin{tabular}{llll}
% 			\toprule
% 			Max. velocity     & $\SI{1.5}{\metre/\second}$       & 3D Map resolution & $\SI{0.1}{\meter}$\\
% 			Max. acceleration & $\SI{1}{\metre/\second^2}$      & Camera resolution & $752\times480$ \\
% 			Max. yaw rate	  & $\SI{0.9}{rad/\second}$         & Max. Connection Distance & $\SI{50}{\metre}$ \\
% 			Max. sensor range & $\SI{4.5}{\metre}$              & Max. Distance from trails & $\SI{8}{\meter}$ \\
% 			\bottomrule
% 		\end{tabular}
% 	}
% 	\caption{Simulation parameters for all presented experiments.}
% 	\label{tab:exp:params}
%     \renewcommand{\arraystretch}{1}
% \end{table}
%

\subsection{Single-robot Experiments}
%
\begin{table}[t!]
	\renewcommand{\arraystretch}{1.2}
	\begin{center}
		\resizebox{0.45\textwidth}{!}{
		\begin{tabular}{l|ccc}
			\toprule
			& Ours & FUEL \cite{zhou2021fuel}\\
			\toprule

			\multicolumn{3}{c}{\textsc{Real Forest}} \\
   
			Completion Time [$\SI{}{\second}$] & \bf{500.7 $\pm$ 14.8} & 757.7 $\pm$ 47.9  \\
			Travelled Distance [$\SI{}{\meter}$] & 645.0 $\pm$ 20.0 & \bf{533.2 $\pm$ 11.0}  \\
			Velocity [$\SI{}{\meter / \second}$] & \bf{1.3 $\pm$ 0.5} & 0.7 $\pm$ 0.4  \\
			\midrule

			\multicolumn{3}{c}{\textsc{Sparse Forest (0.05 trees / }$\SI{}{\meter}^2$)} \\
			Completion Time [$\SI{}{\second}$] & \bf{665.4 $\pm$ 32.7} & 1114.1 $\pm$ 97.4  \\
			Travelled Distance [$\SI{}{\meter}$] & 860.9 $\pm$ 34.0 & \bf{758.1 $\pm$ 57.6}  \\
			Velocity [$\SI{}{\meter / \second}$] & \bf{1.3 $\pm$ 0.6} & 0.7 $\pm$ 0.5  \\
			\midrule

			\multicolumn{3}{c}{\textsc{Average-Density Forest (0.10 trees / }$\SI{}{\meter}^2$)} \\
			Completion Time [$\SI{}{\second}$] & \bf{779.6 $\pm$ 110.9} & 954.1 $\pm$ 28.8 \\
			Travelled Distance [$\SI{}{\meter}$] & 910.3 $\pm$ 63.7 & \bf{713.5 $\pm$ 33.1}  \\
			Velocity [$\SI{}{\meter / \second}$] & \bf{1.2 $\pm$ 0.6} & 0.7 $\pm$ 0.5  \\
			\midrule

			\multicolumn{3}{c}{\textsc{Dense Forest (0.15 trees / }$\SI{}{\meter}^2$)} \\
			Completion Time [$\SI{}{\second}$] & \bf{613.2 $\pm$ 16.2} & 1130.2 $\pm$ 28.8  \\
			Travelled Distance [$\SI{}{\meter}$] & \bf{789.7 $\pm$ 16.8} & 791.0 $\pm$ 37.7  \\
			Velocity [$\SI{}{\meter / \second}$] & \bf{1.2 $\pm$ 0.6} & 0.7 $\pm$ 0.5  \\
			\midrule

			\multicolumn{3}{c}{\textsc{Very Dense Forest (0.20 trees / }$\SI{}{\meter}^2$)} \\
			Completion Time [$\SI{}{\second}$] & \bf{658.2 $\pm$ 57.2} & 904.1 $\pm$ 109.5  \\
			Travelled Distance [$\SI{}{\meter}$] & 802.0 $\pm$ 52.7 & \bf{680.6 $\pm$ 49.9}  \\
			Velocity [$\SI{}{\meter / \second}$] & \bf{1.2 $\pm$ 0.6} & 0.7 $\pm$ 0.5  \\
			%\midrule
			\bottomrule
		\end{tabular}
		}
	\end{center}
	\renewcommand{\arraystretch}{1}
	\caption{Results of the experiments for a single agent. We report the average completion time over 3 runs, as well as the average travelled distance and velocity. The best performance is in bold.}
	\label{table:exp:single}
\end{table}
%
\begin{figure}[t]
	\centering
	\includegraphics[width=0.45\textwidth]{images/experiments/coverage_real_forest_v2.pdf} \vspace{-2mm}
	\caption{Average exploration rate during the experiments in the model \textsc{Real Forest}. The shaded region shows the standard deviation. The proposed method reaches complete coverage in less time than FUEL \cite{zhou2021fuel}.}
	\label{fig:exp:cov_single}
\end{figure}
%
\begin{figure}[t]
	\centering
	\includegraphics[width=0.45\textwidth]{images/experiments/velocity_real_forest_v2.pdf} \vspace{-2mm}
	\caption{The average UAV velocity during the experiments in the \textsc{Real Forest}. The shaded region indicates the standard deviation. The proposed strategy is able to fly the UAV at higher velocities than FUEL. Towards the end of the mission, the UAV following the FUEL strategy also speeds up, as by then the map is mostly explored, and smaller trails are cleared, resembling the Collector mode in the proposed strategy.}
	\label{fig:exp:vel_single}
\end{figure}
%
%
%The high standard deviation in the timings to complete the missions, in particular in the cases of tree densities of $0.10$ and $0.2$ trees/m$^2$, is caused by the complex nature of the map and the large number of occlusions.
%
%
In the single-robot experiments, the models of the synthetic forests are of size $\SI{50}{\meter} \times \SI{50}{\meter} \times \SI{2}{\meter}$, while the 3D reconstruction of the \textsc{Real Forest} has dimensions $\SI{40}{\meter} \times \SI{40}{\meter} \times \SI{2}{\meter}$. 
%
The map resolution is set to $\SI{0.10}{\meter}$.
%
As reported in Table \ref{table:exp:single}, the proposed planner outperforms FUEL \cite{zhou2021fuel} across all scenes in terms of the time taken to complete the mission (Fig. \ref{fig:exp:cov_single}), thanks to our adaptive exploration policy that leads to consistently higher UAV velocity throughout each mission, as illustrated in Fig. \ref{fig:exp:vel_single}.
%, the UAV's velocity generated by our strategy and FUEL during the experiments in \textsc{Real Forest}.
%
These results demonstrate the benefit of using the proposed adaptive exploration strategy over a fixed-mode method.
%
However, notice that the proposed design is less efficient from a global path-planning perspective, leading to longer traveled distances.
%
In fact, decision-making both in Explorer and Collector modes is done on a local-map level, and this may cause the UAV to fly longer routes, deviating from the shortest path.
%
Nonetheless, in the proposed strategy we compensate for this shortcoming by encouraging decisions leading to higher UAV velocities.

%
% Notice also that the high standard deviation of the completion time in some of the experiments, such as the ones with tree density of $0.10$ and $0.2$ trees/m$^2$, is caused by the complex nature of the map and the large number of occlusions.
% %
% In fact, depending on the motion during Exploration mode, numerous trails can be generated, causing the UAV to spend more time in Collector mode.


%
\subsection{Multi-robot Experiments}
%
%In the multi-robot experiments, we show results collected in a range of maps with different topology.
%
%In particular, the proposed planning strategy is tested in models with fixed, homogeneous obstacle density, as well as in randomly generated forests with tree density varying across different regions of the map.
%
In the multi-robot experiments, the proposed planning strategy is tested in a variety of models with fixed, homogeneous obstacle density, as well as in a randomly generated forest with tree density varying across different regions of the map.
%
%In the multi-robot experiments, we utilize models with different sizes and tree densities.
%
%In particular, we show the performance of the proposed approach in diverse maps with fixed and varying obstacle densities across different regions of the area of interest.
%
% \begin{table}[t!]
% 	\renewcommand{\arraystretch}{1.2}
% 	\begin{center}
% 		\resizebox{0.45\textwidth}{!}{
% 		\begin{tabular}{l|ccc}
% 			\toprule
% 			 & Ours & Split Map\\
% 			\toprule

% 			\multicolumn{3}{c}{\textsc{Sparse Forest (0.05 trees / m$\mathbf{^2}$)}} \\
% 			Completion Time [$\SI{}{\second}$]   & \bf{780.3 $\pm$ 32.2} & 834.3 $\pm$ 64.3  \\
% 			Travelled Distance [$\SI{}{\meter}$] & 958.8 $\pm$ 9.2 & \bf{595.7 $\pm$ 51.8}  \\
% 			                                     & 958.7 $\pm$ 60.4 &  \\
% 			Velocity [$\SI{}{\meter / \second}$] & \bf{1.2 $\pm$ 0.6}    & 0.7 $\pm$ 0.4  \\
% 			                                     & \bf{1.3 $\pm$ 0.7}    &  \\
% 			\midrule

% 			\multicolumn{3}{c}{\textsc{Average-Density Forest (0.10 trees / m$\mathbf{^2}$)}} \\
% 			Completion Time [$\SI{}{\second}$]   & \bf{838.5 $\pm$ 64.4} & 848.1 $\pm$ 98.5  \\
% 			Travelled Distance [$\SI{}{\meter}$] & 915.3 $\pm$ 68.4 & \bf{616.1 $\pm$ 40.7}  \\
% 			                                     & 906.2 $\pm$ 58.3 &  \\
% 			Velocity [$\SI{}{\meter / \second}$] & \bf{1.2 $\pm$ 0.5}    & 0.8 $\pm$ 0.4  \\
% 			                                     & \bf{1.1 $\pm$ 0.6}    &  \\
% 			\midrule

% 			\multicolumn{3}{c}{\textsc{Dense Forest (0.15 trees / m$\mathbf{^2}$)}} \\
% 			Completion Time [$\SI{}{\second}$]   & 786.3 $\pm$ 40.7 & \bf{754.0 $\pm$ 23.9}  \\
% 			Travelled Distance [$\SI{}{\meter}$] & 839.0 $\pm$ 26.1 & \bf{586.7 $\pm$ 14.2}  \\
% 			                                     & 882.2 $\pm$ 32.0 &  \\
% 			Velocity [$\SI{}{\meter / \second}$] & \bf{1.2 $\pm$ 0.7}    & 0.8 $\pm$ 0.4  \\
% 			                                     & \bf{1.3 $\pm$ 0.7}    &  \\
% 			\midrule

% 			\multicolumn{3}{c}{\textsc{Very Dense Forest (0.20 trees / m$\mathbf{^2}$)}} \\
% 			Completion Time [$\SI{}{\second}$]   & 803.7 $\pm$ 52.8 & \bf{705.8 $\pm$ 73.2}  \\
% 			Travelled Distance [$\SI{}{\meter}$] & 873.8 $\pm$ 47.0 & \bf{580.3 $\pm$ 73.3}  \\
% 			                                     & 912.6 $\pm$ 42.7 &  \\
% 			Velocity [$\SI{}{\meter / \second}$] & \bf{1.2 $\pm$ 0.7}    & 0.7 $\pm$ 0.5  \\
% 			                                     & \bf{1.2 $\pm$ 0.8}    &  \\
% 			\midrule

% 			\bottomrule
% 		\end{tabular}
% 		}
% 	\end{center}
% 	\renewcommand{\arraystretch}{1}
% 	\caption{Results of the experiments in randomly generated forests with two UAVs. We report the average completion time over 3 runs. We report the average traveled distance and velocity per agent when our strategy is employed. The best performance is in bold.\vspace{-5mm}}
% 	\label{table:exp:multi_2}
% \end{table}
%

\subsubsection{Maps with fixed tree density}
\label{sec:exp:multi:fixed}
%
\begin{figure}[t!]
  \centering
  \includegraphics[width=0.95\linewidth]{images/experiments/exp_two_drones/into_forest_005_two.pdf}
  \caption{Top view of an exploration mission, where a team of two UAVs is tasked to map a randomly generated forest with tree density $0.05$ trees/m$^2$. The initial positions of the UAVs are denoted as colored blobs. For visualization purposes, the UAVs' dimensions are exaggerated, while the map is represented as a 2D occupancy grid obtained by slicing the 3D model at $\SI{1.5}{\meter}$ from the ground.\vspace{-4mm}}
  \label{fig:exp:005_two}
\end{figure}
%
\begin{table}[t!]
	\renewcommand{\arraystretch}{1.2}
	\begin{center}
		\resizebox{0.475\textwidth}{!}{
		\begin{tabular}{l|cc|cc}
			\toprule
			 & Ours & Split Map (FUEL \cite{zhou2021fuel}) & Split Map (Ours)\\
			\toprule

			\multicolumn{4}{c}{\textsc{Sparse Forest (0.05 trees / }$\SI{}{\meter}^2$)} \\
			Completion Time [$\SI{}{\second}$]   & \bf{780.3 $\pm$ 32.2} & 834.3 $\pm$ 64.3      & 620.8 $\pm$ 26.7   \\
			Travelled Distance [$\SI{}{\meter}$] & 958.8 $\pm$ 9.2       & \bf{595.7 $\pm$ 51.8} & 727.3 $\pm$ 29.8  \\
			                                     & 958.7 $\pm$ 60.4      &                       & 770.4 $\pm$ 39.5 \\
			Velocity [$\SI{}{\meter / \second}$] & \bf{1.2 $\pm$ 0.6}    & 0.7 $\pm$ 0.4         & 1.2 $\pm$ 0.6     \\
			                                     & \bf{1.3 $\pm$ 0.7}    &                       & 1.2 $\pm$ 0.5\\
			\midrule

			\multicolumn{4}{c}{\textsc{Average-Density Forest (0.10 trees / }$\SI{}{\meter}^2$)} \\
			Completion Time [$\SI{}{\second}$]   & \bf{838.5 $\pm$ 64.4} & 848.1 $\pm$ 98.5      & 737.6 $\pm$ 47.6  \\
			Travelled Distance [$\SI{}{\meter}$] & 915.3 $\pm$ 68.4      & \bf{616.1 $\pm$ 40.7} & 804.1 $\pm$ 35.9 \\
			                                     & 906.2 $\pm$ 58.3      &                       & 670.0 $\pm$ 93.2 \\
			Velocity [$\SI{}{\meter / \second}$] & \bf{1.2 $\pm$ 0.5}    & 0.8 $\pm$ 0.4         & 1.2 $\pm$ 0.6  \\
			                                     & \bf{1.1 $\pm$ 0.6}    &                       & 1.2 $\pm$ 0.6 \\
			\midrule

			\multicolumn{4}{c}{\textsc{Dense Forest (0.15 trees / } $\SI{}{\meter}^2$)} \\
			Completion Time [$\SI{}{\second}$]   & 786.3 $\pm$ 40.7      & \bf{754.0 $\pm$ 23.9} & 599.4 $\pm$ 26.8 \\
			Travelled Distance [$\SI{}{\meter}$] & 839.0 $\pm$ 26.1      & \bf{586.7 $\pm$ 14.2} & 644.1 $\pm$ 19.2 \\
			                                     & 882.2 $\pm$ 32.0      &                       & 591.4 $\pm$ 135.7 \\
			Velocity [$\SI{}{\meter / \second}$] & \bf{1.2 $\pm$ 0.7}    & 0.8 $\pm$ 0.4         & 1.1 $\pm$ 0.6 \\
			                                     & \bf{1.3 $\pm$ 0.7}    &                       & 1.2 $\pm$ 0.6  \\
			\midrule

			\multicolumn{4}{c}{\textsc{Very Dense Forest (0.20 trees / }$\SI{}{\meter}^2$)} \\
			Completion Time [$\SI{}{\second}$]   & 803.7 $\pm$ 52.8      & \bf{705.8 $\pm$ 73.2} & 641.2 $\pm$ 63.2\\
			Travelled Distance [$\SI{}{\meter}$] & 873.8 $\pm$ 47.0      & \bf{580.3 $\pm$ 73.3} & 607.6 $\pm$ 90.3 \\
			                                     & 912.6 $\pm$ 42.7      &                       & 654.4 $\pm$ 20.5 \\
			Velocity [$\SI{}{\meter / \second}$] & \bf{1.2 $\pm$ 0.7}  &  0.7 $\pm$ 0.5           & 0.8 $\pm$ 0.7 \\
			                                     & \bf{1.2 $\pm$ 0.8}    &                       & 0.9 $\pm$ 0.7 \\
			\midrule

			\bottomrule
		\end{tabular}
		}
	\end{center}
	\renewcommand{\arraystretch}{1}
	\caption{Results in randomly generated forests with fixed tree densities explored with two UAVs, averaged over 3 runs. For the proposed strategy we report the average traveled distance and velocity per agent. For fairness of comparisons, in the last column we report the performance of a variant of our method employed on equally split maps. The best performance is highlighted in bold, without considering the last column.}
	\label{table:exp:multi_2}
\end{table}
%
\begin{figure}[t]
	\centering
	\includegraphics[width=0.45\textwidth]{images/experiments/coverage_multi_005_forest_v2.pdf}
	\caption{Average exploration rate per agent with the proposed approach using two UAVs during the experiments in a random forest with density $0.05$ trees / $m^2$. The shaded region shows the standard deviation. The explored volume is shown to be consistently balanced across the two agents.\vspace{-4mm}}
	\label{fig:exp:cov_multi}
\end{figure}
%
The results of multi-robot collaborative exploration of maps with fixed tree densities with two agents are shown in Table \ref{table:exp:multi_2}, where a maximum connection distance of $\SI{50}{\meter}$ for data exchange between agents is assumed (Fig. \ref{fig:exp:005_two}).
%
Here, experiments are performed in forest models of size $\SI{100}{\meter} \times \SI{50}{\meter} \times \SI{2}{\meter}$ with a map resolution of $\SI{0.10}{\meter}$.
%
%Due to the lack of relevant decentralized planners in the literature, 
The proposed approach is compared against a centralized strategy we devised, employing the FUEL planner \cite{zhou2021fuel} and assigning the UAVs to explore maps of equal sizes (i.e. using map-splitting). 
%
Note that this strategy assumes homogeneous forest maps, and knowledge of the original map size, which renders this unsuitable for realistic deployment unlike the proposed approach; however, comparisons are presented for the sake of benchmarking.
%
For fairness, in the last column of Table \ref{table:exp:multi_2} we also report the performance when using equally split maps with our method as a planning back-end, without considering the communication constraint between agents.
%

%
The proposed strategy reaches comparable results with respect to the centralized approach using FUEL.
%
Similarly to single-robot exploration, the proposed strategy flies the UAVs at higher speeds, incurring longer travel distances.
%
Moreover, our strategy enables automatic load balancing of the exploration mission, yielding similar exploration rates per agent as illustrated in Fig. \ref{fig:exp:cov_multi}.
%
However, in denser forest models, the performance of the proposed approach is seen to degrade, as the UAVs are tasked to fly within a connection range to each other, resulting in limited freedom of movement.
%
This is exacerbated by the increased numbers of obstacles and occlusions in smaller maps, leading to lower exploration rates.
%
Nevertheless, as aforementioned, the proposed approach is realistically deployable in contrast to the baseline strategy using FUEL.
%

\subsubsection{Maps with non-homogeneous tree density}
%
The results of the experiments in a map with non-homogeneous obstacle densities with a team of two agents are shown in Table \ref{table:exp:multi_densities}.
%
We utilize a model with size $\SI{100}{\meter} \times \SI{200}{\meter} \times \SI{2}{\meter}$, with four different tree densities across distinct map regions.
%
The occupancy grip map resolution is set to $\SI{0.15}{\meter}$, with a maximum inter-agent communication distance of $\SI{200}{\meter}$.
%
We perform the same analysis as in Sec. \ref{sec:exp:multi:fixed}, assuming a realistic maximum flight time of $\SI{1500}{\second}$ for the UAVs.
%
As none of the tested planners is able to fully explore the environment within the allowed time, we report the total team coverage at fixed timestamps.
%
% However, since the map to explore are too big in size, we report the coverage at fixed times, assuming a maximum time of $\SI{1500}{\second}$ for the mission, in line with general UAV's battery life.
%
The proposed approach consistently outperforms the solution based on map-splitting using FUEL \cite{zhou2021fuel} as planning back-end.
%
The gain in performance is related to the capacity of our strategy to fly the UAVs faster in regions with lower obstacle density and to explore cautiously more cluttered areas, while clearing smaller frontier trails on the go.
%
This leads to a more efficient exploration process, able to better exploit the capacity of UAVs to perform highly dynamic flights.
%

%
Finally, we report the performance of our method when a team of three robots is deployed.
%
As shown in Table \ref{table:exp:team_size}, a larger team size yields higher total coverage.
%, indicating that the proposed strategy can be extended to large UAVs teams.
%
% However, the gain in having one more robot is not lower than expected, indicating that the proposed coordination strategy has room for improvement.
%
This demonstrates that this work presents an effective strategy for peer-to-peer sharing of the responsibility of exploration of a large forest area, and that the extension to larger teams of multiple UAVs can be realized following this paradigm, pushing for scalable, decentralized multi-robot planning for exploration.
% With this work presenting an effective strategy for peer-to-peer sharing of the responsibility of exploration of a large forest area, the extension to larger teams of multiple UAVs can be realized following this paradigm, pushing for scalable, decentralized multi-robot planning for exploration.
%
% 1. Describe the map and map resolution
% 2. Describe the problem: it is too big, so we collect at key timestamps the coverage
% 3. Analysis with 2 agents: ours is the best and show its benefits compared to the smaller map case. The different densisties imply that our planner can cover the less dense areas faster
% 4. Extension to 3 robots. Indicate that the improvement is not great, indicating that the coordination policy should be improved.
%
% Media:
% - table with key times for the different planners + statistics (or plot)
% - same but 2 and 3

%
\begin{table}[t!]
	\renewcommand{\arraystretch}{1.2}
	\begin{center}
		\resizebox{0.475\textwidth}{!}{
		\begin{tabular}{l|cc|cc}
			\toprule
			 & Ours & Split Map (FUEL \cite{zhou2021fuel}) & Split Map (Ours)\\
			\toprule
			Travelled Distance [$\SI{}{\meter}$] & 1481.9 $\pm$ 467.0       & \bf{735.2 $\pm$ 500.1} &  963.9 $\pm$ 306.5 \\
                                                 & 1487.0 $\pm$ 440.8       & \bf{697.1 $\pm$ 365.6} & 1167.9 $\pm$ 466.4 \\
            %
            & & & \\
            %
			Velocity [$\SI{}{\meter / \second}$] & \bf{1.3 $\pm$ 0.6}        & 0.7 $\pm$ 0.4      & 1.2 $\pm$ 0.6      \\
                                                 & \bf{1.2 $\pm$ 0.7}        & 0.6 $\pm$ 0.5      & 0.8 $\pm$ 0.7      \\
            %
            & & & \\
            % Explored Volume [$\SI{}{\meter}^3$]  & & & \\
            %
		    Explored Volume [$\SI{}{\meter}^3$] - $\SI{300}{\second}$     &     \bf{542.3 $\pm$ 23.3}       &    514.6 $\pm$ 313.0           & 1007.5 $\pm$ 81.5     \\
                                                                          &     565.9 $\pm$ 31.4            &    \bf{632.0 $\pm$ 184.8}      & 947.5 $\pm$ 103.8     \\
            %
            & & & \\
            %
			Explored Volume [$\SI{}{\meter}^3$] - $\SI{600}{\second}$     &     \bf{1062.8 $\pm$ 81.3}      &    840.0 $\pm$ 580.7      & 2043.7 $\pm$ 60.8     \\
                                                                          &     \bf{1011.6 $\pm$ 65.3}      &    728.3 $\pm$ 163.5      & 1679.6 $\pm$ 202.1    \\
            %
            & & & \\
            %
			Explored Volume [$\SI{}{\meter}^3$] - $\SI{900}{\second}$     &     \bf{1400.0 $\pm$ 265.3}     &    1145.3 $\pm$ 814.7    & 2325.6 $\pm$ 183.6    \\
                                                                          &     \bf{1302.6 $\pm$ 110.5}     &    798.8 $\pm$ 146.2     & 2077.1 $\pm$ 486.2    \\
            %
            & & & \\
            %
			Explored Volume [$\SI{}{\meter}^3$] - $\SI{1200}{\second}$    &     \bf{1626.7 $\pm$ 431.2}     &    1330.1 $\pm$ 905.3    & 2571.7 $\pm$ 518.4    \\
                                                                          &     \bf{1466.5 $\pm$ 185.4}     &    910.4 $\pm$ 83.9      & 2450.9 $\pm$ 753.7    \\
            %
            & & & \\
            %
			Explored Volume [$\SI{}{\meter}^3$] - $\SI{1500}{\second}$    &     \bf{1816.0 $\pm$ 550.8}     &    1437.8 $\pm$ 971.8    & 2582.8 $\pm$ 533.8    \\
                                                                          &     \bf{1637.0 $\pm$ 299.1}     &    1040.5 $\pm$ 124.3    & 2578.6 $\pm$ 839.9    \\
			\bottomrule
		\end{tabular}
		}
	\end{center}
	\renewcommand{\arraystretch}{1}
	\caption{Results in a randomly generated forest with non-homogeneous tree densities when explored with two UAVs, averaged over 3 runs. We report the average traveled distance and velocity per agent at $\SI{1500}{\second}$, as well as the total explored volume by the team at different timestamps. In the last column we report the performance of a planning solution using equally split maps with our method as a planning back-end, without considering the communication constraint between agents.
 %In the last column we report the performance of a variant of our method employed on equally split maps. 
 The best performance is highlighted in bold, without considering the last column.
 }
	\label{table:exp:multi_densities}
\end{table}
%
\begin{table}[t!]
	\renewcommand{\arraystretch}{1.2}
	\begin{center}
		\resizebox{0.4\textwidth}{!}{
		\begin{tabular}{c|cc}
			\toprule
        Timestamp & Two Agents & Three Agents \\
			\toprule
        $\SI{300}{\second}$ & $1108.2 \pm \SI{54.7}{\meter^3}$ & \bf{1208.0 $\pm$ 91.6 m$^3$} \\
        & & \\
        $\SI{600}{\second}$ & $2074.3 \pm \SI{144.8}{\meter^3}$ & \bf{2098.4 $\pm$ 143.8 m$^3$} \\
        & & \\
        $\SI{900}{\second}$ & $2702.6 \pm \SI{375.9}{\meter^3}$ & \bf{2748.3 $\pm$ 111.9 m$^3$} \\
        & & \\
        $\SI{1200}{\second}$ & $3093.2 \pm \SI{616.6}{\meter^3}$ & \bf{3223.5 $\pm$ 127.9 m$^3$} \\
        & & \\
        $\SI{1500}{\second}$ & $3453.0 \pm \SI{849.9}{\meter^3}$ & \bf{3621.8 $\pm$ 321.0 m$^3$} \\
			\bottomrule
		\end{tabular}
		}
	\end{center}
	\renewcommand{\arraystretch}{1}
	\caption{Results in a randomly generated forest with varying tree densities across different regions of the model, averaged over 3 runs. Here, the map is explored with teams composed of two and three UAVs. We report the total volume covered by the team at different timestamps. The best performance is highlighted in bold.\vspace{-4mm}}
	\label{table:exp:team_size}
\end{table}
%
